Towards Teachable Autotelic Agents

Autonomous discovery and direct instruction are two distinct sources of learning in children but education sciences demonstrate that mixed approaches such as assisted discovery or guided play result in improved skill acquisition. In the field of Artificial Intelligence, these extremes respectively map to autonomous agents learning from their own signals and interactive learning agents fully taught by their teachers. In between should stand teachable autotelic agents (TAA): agents that learn from both internal and teaching signals to benefit from the higher efficiency of assisted discovery. Designing such agents will enable real-world non-expert users to orient the learning trajectories of agents towards their expectations. More fundamentally, this may also be a key step to build agents with human-level intelligence. This paper presents a roadmap towards the design of teachable autonomous agents. Building on developmental psychology and education sciences, we start by identifying key features enabling assisted discovery processes in child-tutor interactions. This leads to the production of a checklist of features that future TAA will need to demonstrate. The checklist allows us to precisely pinpoint the various limitations of current reinforcement learning agents and to identify the promising first steps towards TAA. It also shows the way forward by highlighting key research directions towards the design or autonomous agents that can be taught by ordinary people via natural pedagogy.

==> abstracts.tex <==
Long : 327 mots

Autonomous discovery and direct instruction are two extreme sources of learning in children, but educational sciences have shown that intermediate approaches such as assisted discovery or guided play resulted in better acquisition of skills. When turning to Artificial Intelligence, the above dichotomy can be translated into the distinction between autonomous agents, which learn in isolation from their own signals, and interactive learning agents which can be taught by social partners but generally lack autonomy. In between should stand \textit{teachable autonomous agents}: agents that learn from both internal and teaching signals to benefit from the higher efficiency of assisted discovery processes. Designing such agents could result in progress in two ways. First, very concretely, it would offer a way to non-expert users in the real world to drive the learning behavior of agents towards their expectations. Second, more fundamentally, it might be a key step to endow agents with the necessary capabilities to reach general intelligence. The purpose of this paper is to elucidate the key obstacles standing in the way towards the design of such agents. We proceed in four steps. First, we build on a seminal work of Bruner to extract relevant features of the assisted discovery processes happening between a child and a tutor. Second, we highlight how current research on intrinsically motivated agents is paving the way towards teachable and autonomous agents. In particular, we focus on autotelic agents, i.e. agents equipped with forms of intrinsic motivations that enable them to represent, self-generate and pursue their own goals. We argue that such autotelic capabilities from the learner side are key in the discovery process. Third, we adopt a social learning perspective on the interaction between a tutor and a learner to highlight some components that are currently missing to these agents before they can be taught by ordinary people using natural pedagogy. Finally, we provide a list of specific research questions that emerge from the perspective of extending these agents with assisted learning capabilities.

BBS : 244 mots (sur 250)

Autonomous discovery and direct instruction are two extreme sources of learning in children, but educational sciences have shown that intermediate approaches such as assisted discovery or guided play resulted in better acquisition of skills. When turning to Artificial Intelligence, the above dichotomy is translated into the distinction between autonomous agents which learn in isolation and interactive learning agents which can be taught by social partners but generally lack autonomy. In between should stand teachable autonomous agents: agents learning from both internal and teaching signals to benefit from the higher efficiency of assisted discovery. Designing such agents would offer a way to non-expert users in the real world to drive their learning behavior towards their expectations. But more fundamentally, it might also be a key step towards general intelligence. In this paper we elucidate obstacles along this research line. First, we build on a seminal work of Bruner to extract relevant features of the assisted discovery processes. Second, we describe current research on autotelic agents, i.e. agents equipped with forms of intrinsic motivations that enable them to represent, self-generate and pursue their own goals. We argue that autotelic capabilities are paving the way towards teachable and autonomous agents. Finally, we adopt a social learning perspective on tutoring interactions and we highlight some components that are currently missing to autotelic agents before they can be taught by ordinary people using natural pedagogy, and we provide a list of specific research questions that emerging from this perspective.

BBS short : 102 mots (sur 100)

Designing teachable and autonomous agents would offer a way to non-expert users to drive their learning behavior towards their expectations, and might be a key step towards general intelligence. In this paper we investigate this research line building on a seminal work of Bruner and on current research on autotelic agents, i.e. agents equipped with intrinsic motivations that enable them to represent, self-generate and pursue their own goals. We then adopt a social learning perspective on tutoring interactions and we highlight key research questions that emerge from the perspective of endowing autotelic agents with the capability to be taught by ordinary people.

BBS short v2 (Hugo) : 

Children are capable of learning both socially and autonomously, a crucial feature that artificial agents currently lack. Designing teachable and autonomous learning agents would offer a way to non-expert users to drive their learning behavior towards their expectations, and might be a key step towards general intelligence. We build on a seminal work of Bruner and on current research on autotelic agents, i.e. agents that generate and pursue their own goals. We then adopt a social learning perspective on tutoring interactions and we highlight key research questions relevant for endowing autotelic agents with the capability to be taught by ordinary people.

Keywords (entre 5 et 10, alphabétique) :

autonomy, autotelic agents, intrinsic motivations, interactive reinforcement learning, social learning, tutoring.

==> commentators.tex <==
Michael Littman      : mlittman@cs.brown.edu
Linda B. Smith       : smith4@indiana.edu
Laura E. Schulz      : lauraelizabethschulz@gmail.com
Joshua B. Tenenbaum  : jbt@csail.mit.edu
Andrea Thomaz        : athomaz@ece.utexas.edu
Tom Ziemke           : tom.ziemke@liu.se
Michael Tomasello    : michael.tomasello@duke.edu
Kerstin Dautenhahn   : kdautenh@uwaterloo.ca
Gergely Csibra       : csibrag@ceu.edu
Dedre Gentner        : gentner@northwestern.edu
Manfred Eppe         : eppe@informatik.uni-hamburg.de
Angelo Cangelosi     : angelo.cangelosi@manchester.ac.uk
Giulio Sandini       : giulio.sandini@iit.it
Felix Hill           : felixhill@google.com
Andy Clark           : Andy.Clark@ed.ac.uk
Jacqueline Gottlieb  : jg2141@columbia.edu
Katharina Rohlfing   : katharina.rohlfing@upb.de
Gianluca Baldassarre : gianluca.baldassarre@istc.cnr.it
Jochen Triesch       : triesch@fias.uni-frankfurt.de
Britta Wrede         : bwrede@techfak.uni-bielefeld.de

==> decstr_description.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{The \decstr experiment}
\label{sec:desctr_exp}

\vspace{3mm}
\par\noindent {\bf The Fetch Manipulate Tutoring Environment}

\begin{figure}[!ht]
  \centering
\vspace{-0.3cm}
{\includegraphics[width=\linewidth]{images/decstr_full-svg.pdf}} \hfill
\vspace{-0.5cm}
   \caption{\textit{The \decstr agent in the Fetch Manipulate Tutoring environment}. \label{fig:env}}
\end{figure}

Need of elementary actions in the physical world

Need to target multiple goals


Experiments with \decstr use the \textit{Fetch Manipulate} environment, a robotic manipulation domain based on \mujoco \cite{todorov2012mujoco}, where a $4$ DoF robotic arm can manipulate blocks around on a table and stack them, as shown in \figurename~\ref{fig:env}. 

The agent does not perceive the environment through images. It is rather equipped with an innate semantic representation of its state as a collection of objects whose position is known, together with a list of all the spatial relations between all pairs of objects in the scene, that we call a spatial configuration. 

The choice to circumvent the processes by which an agent may learn to perceive the world in such a way is based on insights from developmental psychology. Indeed, several authors consider that preverbal infants are equipped very early with object-centered representations \cite{spelke2007core} and a small set of conceptual relational spatial primitives \cite{mandler2012spatial}. These forms of predicates over object relations enable preverbal abstract thoughts and, later on, support early language learning \cite{mandler1999preverbal}.

In the experiments, two of the spatial predicates that infants understand early in their development \cite{mandler2012spatial} are given: the \textit{close} and the \textit{above} binary predicates. 

\vspace{3mm}
\par\noindent {\bf Main results}


The abstract goal layer makes it possible to {\em try again} to address the same goal by targeting a different concrete configuration when a previous attempt with another configuration failed. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Sensorimotor learning architecture and training}


\par {\bf Abstract goal representations}
Beyond perceiving the blocks and their spatial relations, the \decstr agent can set its own goals. These goals merely consist of a spatial configuration which is generally different from the current configuration.
In the experiments described below, goals consist of a vector of 9 binary predicates stating whether one block should be close or away from another, or whether two blocks should be stacked together, specifying which should be above the other.


\par {\bf Sensorimotor learning process}
Equipped with these perceptions and goal representations, the \decstr agent explores the possible spatial configurations by acting on the blocks around. Doing so, it discovers reachable configurations and learns to robustly reproduce them. The agent is not given a repertoire of actions like pushing, dragging, grasping, lifting, moving or releasing, it rather controls the position of the gripper and can open or close it at any moment. But the more semantic actions listed above are reused in many contexts, giving rise for an external observer to a hierarchical interpretation of the behavior of the agent.

To explore the possibilities of its environment, the \decstr agent  sets its own goals based on an automatic curriculum mechanism, starting with random goal configurations. Importantly, in the beginning, it does not know any goal, nor how to reach them: by acting on the blocks, it updates the list of known goals and the probabilities to sample them. 

Besides, to improve its action, it updates its controller based on a reinforcement learning mechanism using two different sources of reward. First, it considers the reward it delivers itself when it reaches its goal. Second, given any trajectory leading to some configuration, it can make "as if" this configuration was its goal and reward itself for reaching it. This mechanism known as "Hindsight Experience Replay" \cite{andrychowicz2017hindsight} has been shown to significantly accelerate learning when reaching a reward is not easy.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Help from a social partner}
\label{sec:intervention}
After a first period of discovering and learning to reach configurations, agents are helped by sporadic interventions of a social partner. Helping the agents in their exploration, the social partner can organize the scene with non-trivial initial configurations.
For instance, the intrinsic exploration mechanisms of the agent may take a lot of time before discovering that blocks can be stacked on top of each other. By organizing initial configurations where blocks are already stacked, the tutor facilitates this discovery. Besides, building a stack of three blocks out of randomly scattered blocks, either in a stack of three blocks or in a pyramid, may be very difficult to the agent. By providing a starting configuration where two blocks are already stacked, or by putting a block in the gripper of the agent, the tutor can strongly facilitate the first achievements of such difficult goals. As the results of \cite{akakzia2020decstr} show, such mechanisms can a lot accelerate the discovery of new goals in the intrinsically motivated agent.

Indeed, by performing ablation experiments where the social partner is removed, \cite{akakzia2020decstr} shows that the discovery of blocks stacking or stacks of three blocks is much faster with the intervention of the tutor.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Language grounding architecture and training}
\label{sec:language}

In a second \textit{language grounding phase}, the social partner describes through language the goals the \decstr agent is achieving. The agent must learn to relate these sentences from the social partner to its newly acquired set of skills, resulting in the sensorimotor grounding of this language input.

For doing so, it trains a language-conditioned goal generation module --~\textit{language module} for short~-- that links language to skills, effectively grounding language in sensorimotor behavior. This language module generates binary configurations matching the agent's current configuration and a sentence describing an expected transformation of one object-pair relation (see \figurename~\ref{fig:schema}). For a given initial configuration and a given sentence, the language module should generate all compatible final configurations, and just these. The \decstr agent is then expected to learn how to reach one of these configurations from the current configuration.

\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.95\linewidth]{images/language_goal_gen.pdf}
   \caption{Language-conditioned policy, goal-conditioned policy and language-conditioned goal generator. Instead of using language to condition policies directly, \decstr uses it to condition a generator of language-agnostic goals.\label{fig:schema}}
\end{figure}

In more details, the set of possible descriptions contains $102$ sentences, each describing, in a simplified language, a positive or negative shift for any of the $9$ predicates corresponding to all spatial relations between all objects (e.g. \textit{get red above green}). At test time, the agent is instructed to change one of the object relations by one of the $102$ sentences. Conditioned on its current configuration and instruction, it samples a compatible goal from the language module and tries to achieve it. 
This \textit{language grounding phase} effectively enables the agent to ground the sentences in its internal representations of its goals and sensorimotor skills. It also account for the fact that the agent may target its own goals or rather follow instructions.

Beyond single instructions, the \decstr agent also performs sequences of instructions or logical combinations of instructions. Indeed, as it can generate a set of goals matching any instruction, it can easily combine these sets to perform logical functions of instructions: \textit{and} is an intersection, \textit{or} is an union and \textit{not} is the complement within the set of goals the agent discovered during sensorimotor training. 
Finally, given sets of compatible goal configurations, the \decstr agent can also \textit{try again}, that is find other target configurations that match the required instruction when previous attempts failed.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Language grounding architecture and training}
\label{sec:language}

In a second \textit{language grounding phase}, the social partner describes through language the goals the \decstr agent is achieving. The agent must learn to relate these sentences from the social partner to its newly acquired set of skills, resulting in the sensorimotor grounding of this language input.

For doing so, it trains a language-conditioned goal generation module --~\textit{language module} for short~-- that links language to skills, effectively grounding language in sensorimotor behavior. This language module generates binary configurations matching the agent's current configuration and a sentence describing an expected transformation of one object-pair relation (see \figurename~\ref{fig:schema}). For a given initial configuration and a given sentence, the language module should generate all compatible final configurations, and just these. The \decstr agent is then expected to learn how to reach one of these configurations from the current configuration.

\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.95\linewidth]{images/language_goal_gen.pdf}
   \caption{Language-conditioned policy, goal-conditioned policy and language-conditioned goal generator. Instead of using language to condition policies directly, \decstr uses it to condition a generator of language-agnostic goals.\label{fig:schema}}
\end{figure}

In more details, the set of possible descriptions contains $102$ sentences, each describing, in a simplified language, a positive or negative shift for any of the $9$ predicates corresponding to all spatial relations between all objects (e.g. \textit{get red above green}). At test time, the agent is instructed to change one of the object relations by one of the $102$ sentences. Conditioned on its current configuration and instruction, it samples a compatible goal from the language module and tries to achieve it. 
This \textit{language grounding phase} effectively enables the agent to ground the sentences in its internal representations of its goals and sensorimotor skills. It also account for the fact that the agent may target its own goals or rather follow instructions.

Beyond single instructions, the \decstr agent also performs sequences of instructions or logical combinations of instructions. Indeed, as it can generate a set of goals matching any instruction, it can easily combine these sets to perform logical functions of instructions: \textit{and} is an intersection, \textit{or} is an union and \textit{not} is the complement within the set of goals the agent discovered during sensorimotor training. 
Finally, given sets of compatible goal configurations, the \decstr agent can also \textit{try again}, that is find other target configurations that match the required instruction when previous attempts failed.
\subsection{Empirical findings}
\par {\bf Sensorimotor Learning Phase: Discovering and Mastering Spatial Configurations}
\label{sec:exp_sensorimotor}

With all the elements described above, the \decstr agent successfully discovers and masters all reachable configurations in its goal space\footnote{Code and videos can be found at \url{https://sites.google.com/view/decstr/}.}. It first masters the easy goals, such as putting blocks close or away to each other. Learning to stack takes more time. Indeed, putting a block above another is more difficult, as it requires the mastery of grasping and releasing the block at the right place. In this process, intervention from the social partner significantly accelerates the training process.

Once getting more expert, the \decstr agent tends to become opportunistic, making profit of the current configuration to reach its goal with as few block moves as possible. 

\par {\bf Grounding language in sensorimotor behavior}
\label{sec:language_results}

After the sensorimotor phase where it decides on its own which goal to target, the \decstr agent is trained during the language grounding phase to learn the meaning of instructions. One can observe that the \decstr agent can generate goals from situations it never encountered, it can generalize the meaning of sentences it never heard and even apply the latter to unknown situations, see \cite{akakzia2020decstr} for more details. 

Finally, the \decstr agent is evaluated on acheiving instructions from the social partner. Three evaluation settings are considered. 

The \textit{transition} setup investigates the average success rate of the agent when asked to perform the $102$ instructions $5$ times each, resetting the environment each time. In the \textit{expression} setup, the agent is evaluated on $500$ randomly generated logical functions of sentences. In both setups, the agent can try $5$ times, enabling it to resample new compatible goals when the previous failed (without reset). The results in Table~\ref{tab:eval} show that the language module efficiently implements language grounding. Agents achieve instructed transitions almost all the time, resampling alternative goals when previous ones failed to reach of success. They only fail when a previous trajectory kicked the blocks out of reach.

\begin{table}[ht!]
\begin{center}
        \caption{Success rates after $1$ and $5$ attempts\label{tab:eval}} 
        \begin{tabular}{l|cccc}\
            Setup & Transition & Expression \\ 
            \hline
            1 attempt & $0.89\pm0.05$ & $0.74\pm0.08$ \\  
            5 attempts & $0.99\pm0.01$ & $0.94\pm0.06$
        \end{tabular}
        \end{center}
\end{table}

Interestingly, in the \textit{expression} setup, when the agent is presented a choice between two instructions, using the \textit{or} operator, it generally chooses the easiest goal to achieve.

Finally, in the \textit{sequence} setup, ten \decstr agents are asked to execute $20$ random sequences of instructions without reset. On average, these agents succeed 15 times before failing.

These results show that endowing the \decstr agent with a set of high level predicates about the scene facilitates a lot the interaction through langage with a human user. Indeed, it is easier for a user to specify goals with these high level predicates, and the agent can implement the specified goal in various ways, making opportunistically profit of the closest elements in the scene, or using variations when its first approach to the goal failed.

==> inquiry.tex <==
current : 1241 mots (target = 1000-2000)

Target article proposal

Title : Towards Teachable Autonomous Agents

We are proposing a paper which aims to stimulate research and discussions at the crossroads of Artificial Intelligence (AI) and cognitive sciences, by taking a developmental perspective on the design of artificial learning agents. Our starting point is the fact that, in the current AI literature, two apparently irreconcilable research lines coexist: one that focuses on autonomous agents, which learn in isolation from their own signals, and interactive learning agents which can be taught by social partners but generally lack autonomy. We hypothesize that the current lack of an integrated theoretical perspective between these approaches is a major obstacle towards scaling up AI to human-like intelligence. Leveraging developmental human sciences and the emerging domain of developmental AI, we address this issue by proposing a novel theoretical framework.

In cognitive and educational sciences, these two lines are actually reconciled by the "assisted discovery" or "guided play" approaches to education [Yu et al., 2018], where children learn on their own under the guidance of a tutor. This perspective about tutoring is central in the work of Jerome Bruner, a psychologist from which we draw inspiration, as well as in the work of Lev Vygostky who showed that autonomy and sociality are integrated and build on each other in the processes that lead to the development of human intelligence [Wood et al., 1973, Vygotsky, 1978].

So, in AI, between autonomous agents and interactive learning agents should stand \textit{teachable autonomous agents}: agents that learn from both internal and teaching signals to benefit from the higher efficiency of assisted discovery processes. Designing such agents could result in progress in two ways. First, very concretely, it would offer a way to non-expert users in the real world to drive the learning behavior of agents towards their expectations. Second, more fundamentally, it might be a key step to endow agents with the necessary capabilities to reach general intelligence. The purpose of our paper is to elucidate the key obstacles standing in the way towards the design of such agents. 

Our most important message is that, in order to solve the apparent contradiction between the design requirements of autonomous agents and interactive learning agents, we should consider autotelic agents, i.e. agents equipped with forms of intrinsic motivations that enable them to represent, self-generate and pursue their own goals. We stress that leveraging recent work on autotelic agents in AI [Colas et al., 2019, 2020, Akakzia et al. 2021] makes it possible to model the tutoring processes studied by Bruner and to deeply rethink the interaction between a human tutor and a learning agent. In particular, we argue that such autotelic capabilities from the learner side are key in the discovery process, in accordance with recent studies on the importance of play and curiosity in cognitive processes [Chu&Schulz, 2020]. Beyond that, we claim that these autotelic capabilities are also crucial to enable the agent to learn to interpret and respond to goal-related signals emitted by tutors and social partners.

From that starting point, we adopt a social learning perspective on the interaction between a tutor and a learner to highlight some components that are currently missing to interactive reinforcement learning agents and autotelic agents before they can be taught by ordinary people using natural pedagogy. 

We consider social learning as a mutual exchange between the tutor and the learner exploiting two channels: a task channel used to communicate through the task as tutor usually do with demonstrations or learners to demonstrate their current mastery, and a more social, direct interaction channel used for verbal and nonverbal communication like directing attention, providing feedback and requesting actions from both sides.  Based on this framework, we outline the need for arbitration mechanisms that let the agent engage into or disengage from interactions with the tutor. We also outline that these autotelic agents need a theory of mind to achieve the richness of human social learning, as also pointed out in [Velez and Gweon, 2021]: we argue that their capacity to represent and manipulate their own goals to understand the goal of others should be key to understand the tutor's intent and to appropriately emit transparency feedback signals about their current understanding of the tutoring situation. Finally, we provide a list of specific open research questions that emerge from the perspective of extending autotelic agents with the social learning capabilities that we have highlighted. We argue that this research perspective opens potential high impact not only in AI, but also back to psychology.

Like the recent perspective paper from Lake et al. [2017], our target paper highlights the importance of grounding AI within a better understanding of some fundamental human cognitive processes. However, Lake et al. focus mostly on statistical learning and overlook both reinforcement learning and autotelic mechanisms, as well as their interaction with social learning, which play a crucial role in the cognitive development of children. The work of [Velez&Gweon, 2021] is closer to ours, as it takes a developmental stance and it assigns a key role to reinforcement learning in the developmental process. But Velez&Gweon stick to the external reward perspective of interactive reinforcement learning, and as such cannot account for the role of self-generating and pursuing goals in the cognitive development of children, whose importance was outlined in [Chu&Schulz, 2020].

To conclude, we believe our work is important for two reasons. First, we think it addresses some of the key shortcomings of current approaches to AI which heavily rely on external rewards, limiting current capacities to develop artificial systems with human-like intelligence. Second, we argue that in a world where AI systems are increasingly involved in interaction with humans, the ability to teach autonomous agents through natural social interaction, such as in the normal process of education of human children, will be of key importance.

References :

[Akakzia et al., 2021] Akakzia, A., Colas, C., Oudeyer,  P.-Y., Chetouani,  M., Sigaud, O., 2021. Grounding language to autonomously-acquired skills via goal generation. In: ICLR 2021-Ninth International Conference on Learning Representation. pp. 1–21.

[Chu&Schulz, 2020] Chu, J., Schulz, L. E., 2020. Play, curiosity, and cognition. Annual Review of Developmental Psychology 2, 317–343.

[Colas et al., 2019] Colas, C., Oudeyer, P.-Y., Sigaud, O., Fournier, P., Chetouani, M., 2019. CURIOUS: Intrinsically motivated multi-task,  multi-goal  reinforcement learning. In:  International Conference on Machine  Learning (ICML). pp. 1331–1340.

[Colas et al., 2020] Colas, C., Karch, T., Lair, N., Dussoux, J.-M., Moulin-Frier, C., Dominey, P. F., Oudeyer, P.-Y., 2020. Language as a cognitive tool to imagine goals in curiosity-driven exploration. Advances in Neural Information Processing Systems 33 (NeurIPS 2020).

[Lake et al., 2017] Lake, B. M., Ullman, T. D., Tenenbaum, J. B., Gershman, S. J.,  2017. Building machines that learn and think like people. Behavioral and Brain Sciences 40.

[Velez&Gweon, 2021] Velez, N., Gweon, H., 2021. Learning from other minds: An optimistic critique of reinforcement learning models of social learning. Current Opinion in Behavioral Sciences 38:110–115.

[Vygotsky, 1978] Vygotsky,  L. S.,  1978. Tool and Symbol in Child Development. In:  Mind in Society. Harvard University Press, Ch. Tool and Symbol in Child Development, pp. 19–30.

[Wood et al., 1973] Wood, D., Bruner, J. S., Ross, G., 1976. The role of tutoring  in  problem  solving.  Journal  of  child  psychology  and psychiatry 17 (2), 89–100.

[Yu, Y., Shafto, P., Bonawitz, E., Yang, S. C. H., Golinkoff, R. M., Corriveau, K. H., ... & Xu, F., 2018]. The theoretical and methodological opportunities afforded by guided play with young children. Frontiers in psychology, 9, 1152.

==> more_cognitive_challenges.tex <==

\subsection{More general goal understanding}

\cite{kaplan2006challenges,tomasello2005understanding,dawson2004early}

Whereas goals sentences presented to the \decstr agent directly consist of block manipulation instructions, in \cite{wood1976role}, goals are specified to the agent rather indirectly. The tutor can ask the agent either to compare two block configurations to outline that the just produced configuration is erroneous, or to produce "more of the same" configuration. 

Being capable to interpret such goals requires some capabilities to mentally compare two configurations, to generalize from one configuration to another or even to abstract away what is common to several configurations to be able to build new ones that share the same abstract properties.

In other terms, the agent should be capable of manipulating in a richer way the abstract representations that the \decstr agent is sketching as a pair of simple spatial predicates. Beyond this simple extension of representational manipulation capabilities, this line of thoughts is pointing towards the necessity of endowing teachable autonomous agent with {\em common sense} so that the can interact more fluidly with social partners \cite{shanahan2020artificial}.

\subsection{Gaze following, Joint attention, Mutual engagement}

Necessity of attention to avoid the huge combinatorial of potential goals.

% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % 
% Towards sharing representations
% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % 

\subsection{Teaching to share representations}

\todo{This is more in the language grounding side, thus absent from \cite{wood1976role}}

The developmental trajectory of an agent might be influenced by making so that its representations evolve towards those of its tutor.

To represent the current configuration of objects around, the \decstr agent uses two given predicates, close and above. In the case of those predicate, it is debated whether babies are born with them \cite{spelke2007core} or acquired through experience \cite{mandler2012spatial}. At least, we may consider that we are endowed with inductive biases that make so that any human (and probably also many animals) will learn about being close and being above without intervention of a tutor. So tutoring may not be necessary for the acquisition of such predicates.

In the case of the \decstr experiments, as the predicates are given, the role of the language learning part is limited to learning that some words refer to specific blocks, some words describe an action and some words correspond to the predicates whose meaning in terms of current or goal configuration is already mastered by the agent. For learning this correspondence, the \decstr agents calls upon a language-conditioned goal generator, as depicted in \figurename~\ref{fig:fetch_env}.

So here tutoring is not about the acquisition of the right predicates, but about establishing the right correspondence between learned predicates and given sentences.

But for the acquisition of more complex representations or predicates, tutoring does certainly play a role. It is probably one of the central role of school in our societies to convey the adequate environment to acquire the complex representations and concepts that are at the heart of the various disciplines that are commonly studied all over the world.

So, to get teachable agents, we would like to endow them with the mechanisms that make it possible for a human tutor to enrich their representations with new predicates. 

To stay close to the domain covered in \cite{akakzia2020decstr} and \cite{wood1976role}, let us take the example of the acquisition of the concept of pyramid, which can be made concrete by building a pyramid of blocks.

By which ways can a tutor teach the agent the predicate being a pyramid?

The tutor can wait that the agent builds a pyramid by chance. He or she can also organize the environment in a configuration close to a pyramid, instruct the agent with a local goal that will complete the pyramid. He or she can finally build pyramids directly, to increase the probability of occurrence of this configuration. In all cases, he or she should utter the word “pyramid” when it is done.  

We are then in the situation of a language guessing game \cite{steels2001language}, but where the reference is not about an object but about a complex set of spatial relations between objects.

In this situation, all the previously described mechanisms can also play a role.

Gaussian Process Classifiers \cite{kulick2013active}

VQ-VAE \cite{van2017neural}

Get the symbolic representation from images \cite{asai2019unsupervised}
 
\subsection{Towards more advanced language-based cognitive capabilities}


Being able to imagine new goals by leveraging the flexibility of language could be one of these crucial capabilities that an agent should have to become intelligent in a strong sense, fleshing out the general perspective of \cite{bruner1990acts,bruner2009culture} that cultural interaction plays a key role in the development of our cognitive capabilities.



==> orcid_authors.tex <==
Olivier Sigaud : 0000-0002-8544-0229
Ahmed Akakzia : 0000-0001-8638-2107
Mohamed Chetouani : 0000-0002-2920-4539
Hugo Caselles-Dupré : 0000-0003-2711-5732
Cédric Colas : 0000-0003-0212-427X
Pierre-Yves Oudeyer : 0000-0002-1277-130X

==> rationale.tex <==
358 mots (on a droit à 500 mots)

Our paper aims to stimulate research and discussions at the crossroads of AI and cognitive sciences, by taking a developmental perspective on the design of artificial learning agents. Our starting point is the fact that, in the current AI literature, two apparently irreconcilable research lines coexist: one that focuses on autonomous agents which learn on their own, and one that focuses on teaching agents from external reward signals. In cognitive and educational sciences, these two lines are actually reconciled by the "assisted discovery" or "guided play" approaches to education, where children learn on their own under the guidance of a tutor. This perspective about tutoring is central in the work of Jerome Bruner, a psychologist from which we draw inspiration, as well as in the work of Lev Vygostky who showed that autonomy and sociality are integrated and build on each other in the processes that lead to the development of human intelligence.
Leveraging recent advances in AI that consider autotelic agents, i.e. agents equipped with forms of intrinsic motivations that enable them to represent, self-generate and pursue their own goals, we are offering a framework which makes it possible to model the tutoring processes studied by Bruner and to deeply rethink the interaction between a human tutor and a learning agent.

This work is important for two reasons. First, we think it addresses some of the key limits of current approaches to AI who heavily rely on external rewards, limiting current capacities to develop artificial systems with human-like intelligence. Second, we argue that in a world where AI systems are increasingly involved in interaction with humans, the ability to teach autonomous agents through natural social interaction, such as in the normal process of education of human children, will be of key importance.

 Thus, from a broader perspective, and by leveraging work from developmental psychology, this paper identifies key limits of current AI approaches to enable human-like intelligence. From this standpoint, we then describe a novel research program associated to recent emerging works that begin to address these limits. We argue that this research perspective opens potential high impact not only in AI, but also back in psychology.





